Accounting for Sycophancy in Language Model Uncertainty Estimation

Effective human-machine collaboration requires machine learning models to externalize uncertainty, so users can reflect and intervene when necessary. For language models, these representations of uncertainty may be impacted by sycophancy bias: proclivity to agree with users, even if they are wrong. For instance, models may be over-confident in (incorrect) problem solutions suggested by a user. We study the relationship between sycophancy and uncertainty estimation for the first time. We propose a generalization of the definition of sycophancy bias to measure downstream impacts on uncertainty estimation, and also propose a new algorithm (SyRoUP) to account for sycophancy in the uncertainty estimation process. Unlike previous works on sycophancy, we study a broad array of user behaviors, varying both correctness and confidence of user suggestions to see how model answers (and their certainty) change. Our experiments across conversation forecasting and question-answering tasks show that user confidence plays a critical role in modulating the effects of sycophancy, and that SyRoUP can better predict these effects. From these results, we argue that externalizing both model and user uncertainty can help to mitigate the impacts of sycophancy bias.

==> latex/04_results_old.tex <==




\begin{table*}[]
\centering\small
\begin{tabular}{lllllllllllll}
\toprule
& \multicolumn{2}{l}{Llama 3.1 8B} & \multicolumn{2}{l}{Llama 3.1 70B} & \multicolumn{2}{l}{Mistral v0.3 7B} & \multicolumn{2}{l}{Mixtral 8x22B} & \multicolumn{2}{l}{Qwen 72B} & \multicolumn{2}{l}{mean \textbf{ACC}} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
\textbf{uncertainty} & \xmark               & \checkmark           & \xmark              & \checkmark             & \xmark               & \checkmark              & \xmark              & \checkmark             & \xmark            & \checkmark   & \xmark            & \checkmark        \\\midrule
\texttt{wiki}        & 67.5             & 68            & 64              & 62              & 51.5             & 54               & 53              & 58              & 53.5          & 54.5  & 57.9	& \textbf{59.3}       \\
\texttt{reddit}      & 58               & 57.5          & 66.5            & 61.5            & 52               & 51.5             & 54              & 59.5            & 43.5          & 48.5         & 54.8	&\textbf{55.7} \\
\texttt{casino}      & 60               & 65            & 70.5            & 67.5            & 37.5             & 45.5             & 64.5            & 69              & 63            & 66.5        & 59.1	& \textbf{62.7} \\
\texttt{donations}   & 58               & 57.5          & 57.5            & 55.5            & 61.5             & 58.5             & 58.5            & 53.5            & 61            & 61.5         & 59.3	& 57.3\\\midrule
mean \textbf{ACC}   &  60.88	&\textbf{62.00}	&64.63	&61.63	&50.63	&\textbf{52.38}	&57.50	&\textbf{60.00}	&55.25	&\textbf{57.75}	&57.78	&\textbf{58.75}\\\bottomrule      
\end{tabular}
\caption{Accuracy of models at conversation forecasting with (\checkmark) or without (\xmark) uncertainty-aware prompting strategy. \textbf{Bold} shows improvement from incorporating uncertainty, for both model and data averages.}
\label{tab:acc}
\end{table*}
%
\begin{table*}[]
\centering\small
\begin{tabular}{lllllllllllll}
\toprule
& \multicolumn{2}{l}{Llama 3.1 8B} & \multicolumn{2}{l}{Llama 3.1 70B} & \multicolumn{2}{l}{Mistral v0.3 7B} & \multicolumn{2}{l}{Mixtral 8x22B} & \multicolumn{2}{l}{Qwen 72B} & \multicolumn{2}{l}{mean \textbf{F1}} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
\textbf{uncertainty} & \xmark               & \checkmark           & \xmark              & \checkmark             & \xmark               & \checkmark              & \xmark              & \checkmark             & \xmark            & \checkmark   & \xmark            & \checkmark        \\\midrule
\texttt{wiki}        & 0.692	&0.698	&0.621	&0.600	&0.185	&0.258	&0.266	&0.400	&0.243	&0.305	&0.401	&\textbf{0.452}       \\
\texttt{reddit}      & 0.702	& 0.699	& 0.747	& 0.712	& 0.461	& 0.497	& 0.494	& 0.610	& 0.199	& 0.383	& 0.521	& \textbf{0.580} \\
\texttt{casino}      & 0.722	& 0.776	& 0.817	& 0.804	& 0.302	& 0.586	& 0.719	& 0.800	& 0.750	& 0.791	& 0.662	& \textbf{0.751} \\
\texttt{donations}   & 0.664	& 0.647	& 0.677	& 0.664	& 0.696	& 0.661	& 0.664	& 0.654	& 0.639	& 0.664	& 0.668	& 0.658\\\midrule
mean \textbf{F1}   &  0.695	&\textbf{0.705}	&0.716	&0.695	&0.411	&\textbf{0.500}	&0.536	&\textbf{0.616}	&0.458	&\textbf{0.536}	&0.563	&\textbf{0.610}\\\bottomrule      
\end{tabular}
\caption{F1 score of different models at conversation forecasting with (\checkmark) and without (\xmark) uncertainty-aware prompting strategy. \textbf{Bold} shows improvement from incorporating uncertainty for model/data averages.}
\end{table*}
\label{tab:f1}
%
\paragraph{Metrics} We report the accuracy \textbf{ACC} and \textbf{F1} score of the CoT predictions, along with the evaluations for explanation quality described in \S~\ref{sec:meth}. These are often averaged across models or datasets. Generally, we use Hoeffding's Inequality to test for statistical significance of the averages we report. It is a conservative bound, but lacks distributional assumptions, allowing us to apply it to the micro-averages we report. We use a significance level $\alpha = 0.05$ without any Bonferroni correction.
\paragraph{Setup} We use Mistral 7B v0.3 and Mixtral 8x22B \citep{jiang2023mistral, jiang2024mixtral}, Qwen2 72B \citep{yang2024qwen2}, and Llama 3.1 8B and 70B \citep{llama3modelcard}. We use default hyper-parameters for Llama, from the official GitHub repository (temp = 0.6, top p = 0.9). For other models, we use temp = 0.7 and top p = 1. We run inference with \href{https://together.ai}{together AI}.
\subsection{Uncertainty and CoT Prediction Accuracy}
\begin{displayquote}
\textit{RQ1: Does uncertainty-aware CoT increase accuracy compared to standard CoT?} \\
\textit{A: There may be a slight positive increase, but results are not statistically significant or consistent.}
\end{displayquote}
\paragraph{CoT Accuracy} Table~\ref{tab:acc} shows accuracy of CoT forecasting with and without consideration of uncertainty for all datasets and models. Averages show that different models experience slight changes in performance with/without the use of uncertainty estimates for inference. Changes in accuracy range between 1 and 3\% when looking at individual model performance (averaged across data). When looking at performance on individual datasets, changes are similar. Although no results are statistically significant, we observe that more often than not, data/model averages show a slight increase in accuracy.
\paragraph{CoT F1 Score} Table~\ref{tab:f1} shows F1 scores of CoT forecasting with and without consideration of uncertainty. Results echo trends discussed in the previous paragraph, but when increases in F1 score do occur for uncertainty-aware CoT, the magnitude of increase seems to be higher. For instance, for individual models, the average F1 increases near 0.1 points (on a 0-1 scale). This trend also holds for some datasets, with \texttt{casino} experiencing a relatively high increase in F1 score (using uncertainty estimates for inference).
\paragraph{Discussion} Findings indicate no statistically significant changes in accuracy when using uncertainty estimates for inference, in place of traditional CoT. Yet, there is a some noticeable increase in average accuracy for most models and datasets. Moreover, when one considers accuracy under data imbalance (i.e., measured by F1 scores) changes in the magnitude of scores are larger, with uncertainty-aware CoT showing positive performance gains. This suggests \textit{uncertainty-aware inference may have a particular positive benefit when outcomes have a biased base rate of occurrence}. For instance, in \texttt{casino}, most users are satisfied with their deal, leading to a base rate near 80\%. At the same time, we do not test significance of these results (Hoeffding is not applicable). Overall, our takeaway from these results is that uncertainty-aware CoT tends to offer no significant changes in forecasting performance,  but can offer some performance improvement in certain scenarios (e.g., imbalanced data or specific models).
%
\begin{table*}[]
\centering\small
\begin{tabular}{lllllllllllll}
\toprule
& \multicolumn{2}{l}{Llama 3.1 8B} & \multicolumn{2}{l}{Llama 3.1 70B} & \multicolumn{2}{l}{Mistral v0.3 7B} & \multicolumn{2}{l}{Mixtral 8x22B} & \multicolumn{2}{l}{Qwen 72B} & \multicolumn{2}{l}{mean \textbf{FUB}} \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
\textbf{uncertainty} & \xmark               & \checkmark           & \xmark              & \checkmark             & \xmark               & \checkmark              & \xmark              & \checkmark             & \xmark            & \checkmark   & \xmark            & \checkmark        \\\midrule
\texttt{wiki}        & 0.16	& 0.165	& 0.315	& 0.15	& 0.215	& 0.195	& 0.395	& 0.355	& 0.435	& 0.36	& 0.304	& 0.245*      \\
\texttt{reddit}      & 0.125	&0.14	&0.1	&0.035	&0.02	&0.025	&0.135	&0.12	&0.32	&0.25	&0.14	&0.114 \\
\texttt{casino}      & 0.095	&0.515	&0.26	&0.12	&0.04	&0.125	&0.035	&0.245	&0.18	&0.26	&0.122	& \textbf{0.253}* \\
\texttt{donations}   & 0.27	&0.165	&0.38	&0.24	&0.16	&0.195	&0.2	&0.31	&0.39	&0.32	&0.28	&0.246\\\midrule
mean \textbf{FUB}   &  0.16	&\textbf{0.25}*	&0.26	&0.14*	&0.11	&\textbf{0.14}	&0.19	&\textbf{0.26}*	&0.33	&0.30	&0.21	&0.21\\\bottomrule      
\end{tabular}
\caption{Faithfulness  upperbound of model explanations while forecasting conversation outcomes with (\checkmark) and without (\xmark) uncertainty-aware prompting strategy. \textbf{FUB} ranges between 0 and 1 where higher scores mean the model was likely to give faithful explanations, even when its sycophancy bias was exploited. \textbf{Bold} shows improvement from incorporating uncertainty for model/data averages. An asterisk is used to indicate if increases/decreases in results are statistically significant.}
\label{tab:faith}
\end{table*}
\subsection{Uncertainty and CoT Explanation Quality}
\begin{displayquote}
    \textit{RQ2: Does explanation quality improve when using uncertainty-aware CoT?} \\
    \textit{A: Possibly. While one evaluation protocol suggest this is the case (more often than not), another indicates quality changes are more specific to the model and dataset studied.}
\end{displayquote}
\paragraph{Explanation Win Rates} Table~\ref{tab:winrates} shows the win rates (as judged by GPT-4o mini) using the evaluation criteria described in \S~\ref{sec:meth}. For all datasets and all models, more often than not, uncertainty-aware CoT beats traditional CoT in terms of the explanation quality criteria. Frequently, these results are statistically significant as well. The uncertainty-aware win rates tend to be highest for larger models (Llama 3.1 70B and Qwen2 72B). Also, when win rates are greater than 50\% for one criteria, they tend to be greater than 50\% for all criteria (and vice versa). The highest average win rates come from the criteria of clarity and leverage (i.e., recall the latter is the ability to sway one's opinion). Average win rates for the other criteria are not statistically significant. 
\begin{table}
\centering\small
\begin{tabular}{lllllll}
\toprule
\textbf{model}                            & \textbf{data}      & \textbf{QR}   & \textbf{AR}   & \textbf{CL}   & \textbf{LV}   & \textbf{avg}  \\\midrule
\multirow{4}{1cm}{Llama 3.1 70B}   & \texttt{wik.}      & 0.57 & 0.62 & 0.63 & 0.66 & \textbf{0.62}* \\
                                 & \texttt{cas.}    & 0.62 & 0.59 & 0.69 & 0.70 & \textbf{0.65}* \\
                                 & \texttt{red.}    & 0.59 & 0.57 & 0.63 & 0.68 & \textbf{0.61}* \\
                                 & \texttt{don.} & 0.63 & 0.61 & 0.68 & 0.69 & \textbf{0.65}* \\\midrule
\multirow{4}{1cm}{Llama 3.1 8B}    & \texttt{wik.}      & 0.63 & 0.60 & 0.62 & 0.64 & \textbf{0.62}* \\
                                 & \texttt{cas.}    & 0.55 & 0.53 & 0.55 & 0.63 & \textbf{0.56}* \\
                                 & \texttt{red.}    & 0.60 & 0.56 & 0.62 & 0.66 & \textbf{0.61}* \\
                                 & \texttt{don.} & 0.51 & 0.53 & 0.53 & 0.57 & \textbf{0.53} \\\midrule
\multirow{4}{1cm}{Mistral v0.3 7B} & \texttt{wik.}      & 0.44 & 0.39 & 0.44 & 0.45 & 0.43* \\
                                 & \texttt{cas.}    & 0.56 & 0.57 & 0.61 & 0.59 & \textbf{0.58}* \\
                                 & \texttt{red.}    & 0.44 & 0.35 & 0.38 & 0.45 & 0.40* \\
                                 & \texttt{don.} & 0.50 & 0.55 & 0.51 & 0.53 & \textbf{0.52} \\\midrule
\multirow{4}{1cm}{Mixtral 8x22B}   & \texttt{wik.}      & 0.50 & 0.42 & 0.47 & 0.49 & 0.47 \\
                                 & \texttt{cas.}    & 0.51 & 0.48 & 0.59 & 0.51 & \textbf{0.52} \\
                                 & \texttt{red.}    & 0.40 & 0.37 & 0.36 & 0.38 & 0.38* \\
                                 & \texttt{don.} & 0.50 & 0.48 & 0.49 & 0.51 & 0.49 \\\midrule
\multirow{4}{1cm}{Qwen2 72B}       & \texttt{wik.}      & 0.56 & 0.65 & 0.66 & 0.77 & \textbf{0.66}* \\
                                 & \texttt{cas.}    & 0.70 & 0.62 & 0.74 & 0.79 & \textbf{0.71}* \\
                                 & \texttt{red.}    & 0.61 & 0.63 & 0.67 & 0.74 & \textbf{0.66}* \\
                                 & \texttt{don.} & 0.56 & 0.52 & 0.59 & 0.66 & \textbf{0.58}* \\\midrule
    \textbf{avg}                         &   & \textbf{.55}	&\textbf{.53}	&\textbf{.57}*	&\textbf{.60}*\\\bottomrule
\end{tabular}
\caption{Win rates for explanations generated via uncertainty-aware CoT, compared to explanations generated via traditional CoT. Rater criteria is described in \S~\ref{sec:meth}. Average win rates higher than 50\% are \textbf{bold}, indicating uncertainty-aware CoT beat traditional CoT more often than not. Asterisks indicate if an (averaged) win rate is statistically higher/lower than 50\%.}
\label{tab:winrates}
\end{table}
\begin{table}
\centering\small
\begin{tabular}{llllll}
\toprule
          & \textbf{QR}    & \textbf{AR}   & \textbf{CL}   & \textbf{LV}    & \textbf{avg}   \\\midrule
\texttt{wiki}      & -0.05 & 0.00 & 0.00 & -0.03 & -0.02 \\
\texttt{casino}    & 0.02  & \textbf{0.07} & 0.05 & \textbf{0.09}  & 0.07  \\
\texttt{reddit}    & \textbf{0.08}  & \textbf{0.13} & \textbf{0.12} & \textbf{0.12}  & 0.13  \\
\texttt{donations} & 0.06  & \textbf{0.07} & 0.04 & 0.05  & 0.07 \\\midrule
\textbf{avg} & 0.03 & 0.07 & 0.05 & 0.06 & \\
\bottomrule
\end{tabular}
\caption{Linear correlation between win rates and the log sequence probability of the model response (i.e., computed with the token logits). \textbf{Bold} shows correlations that are significant using a $t$-test at level $\alpha=0.05$.}
\label{tab:cor}
\end{table}
%
\paragraph{Sycophancy Tests for Faithfulness}
Table~\ref{tab:faith} shows the results of faithfulness tests, where the prompt is modified to exploit the sycophancy bias of LLMs (see \S~\ref{sec:meth}, \textbf{FUB}). The metric reported is the faithfulness upperbound, which is precisely the accuracy of the model when subject to this prompt bias. Results are mixed, showing that for some models/datasets uncertainty-aware CoT exacerbates sycophancy bias (and subsequent unfaithfulness of the explanations). For other models/datasets, it actually improves faithfulness of explanations. Notably this behavior is not consistent across model sizes or model families. For instance, Llama 3.1 8B is improved by considering uncertainty, while its 70B counterpart is negatively impacted. Other large models (like Mixtral 8x22B) are positively impacted. Meanwhile, many of these results are statistically significant, re-enforcing that performance impact is truly a ``mixed bag'' dependent on the model, rather than some artifact of random chance. The behavior is also not consistent across conversation settings. One negotiation dataset exhibits statistically significant improvement (\texttt{casino}) when uncertainty-aware CoT is used, while the other (\texttt{donations}) exhibits moderate degradation. When the outcome is predicting a personal attack (\texttt{wiki} and \texttt{reddit}), uncertainty-aware CoT does appear to worsen susceptibility to the sycophancy bias (and thus, worsen faithfulness).
\paragraph{Discussion}
Findings show that uncertainty-aware CoT tends to improve the clarity and leverage of model explanations fairly consistently (i.e., where leverage is the ability to convince). These results were statistically significant. We suspect that question relevance and answer relevance had insignificant differences in win rates (with/without uncertainty estimation) because these criteria were under-specified. Indeed, most information provided by a model would be ``relevant,'' unless the explanation was very off topic. One additional issue with the interpretation of answer relevance was the fact that the rater model did not have access to the original system prompt for forecasting (which may have specified important details about the interpretation of the answer). Nonetheless, our analysis does reveal certain aspects of explanation quality are increased as a result of incorporating uncertainty in the model inference. Meanwhile, no aspects measured by the rater were consistently and significantly decreased. \textit{One alarming finding is the susceptibility of all language models to sycophancy bias} (and thus, unfaithful explanation). Comparing accuracy before/after interjection of the sycophancy biased input highlights this problem. This sycophancy bias is not consistently resolved by any strategy we employ, leaving the problem as an area of future work. On some datasets (\texttt{casino}), consideration of uncertainty in CoT does offer significant improvement, suggesting our proposal may be a promising strategy in specific scenarios.
\subsection{Internal Model Confidence and Explanation Quality}
\paragraph{Correlation Analysis} 
Table \ref{tab:cor} shows linear (Pearson) correlation between the (log) sequence probability assigned by the model (when using uncertainty-aware CoT) and this same model’s win rates for each quality criteria. For the Reddit corpus, all aspects of explanation quality have positive correlation with the model’s sequence probability (this is statistically significant). This means that log sequence probability has a noisy linear relationship with the explanation quality for this data. Other notable (significant) correlations are between log sequence probability and answer relevance (on donations and casino) as well as leverage (on casino). On average, answer relevance had the highest correlation with log sequence probability. Leverage had the second highest correlation.
\paragraph{Discussion}
This analysis shows a slightly different perspective of “confidence” than we have focused on thus far. Specifically, looking at model confidence in the explanation itself and the correlation of this confidence with the explanation quality. Interestingly, model confidence -- as measured by token logits -- \textit{does} appear to correlate with answer quality, at least for some specific datasets and evaluation criteria. This fact suggests a potential avenue for unsupervised explanation evaluation; e.g., in deciding whether to show or trust an explanation at deployment. Still, the correlation is weak (and often non-existent, for some datasets), suggesting models can still be “confidently wrong” in their explanations. As noted, answer relevance was most correlated with sequence probability. One possible explanation is the fact that all measured probabilities are conditional on previous text. Thus, explanations which are more likely given an answer (or vice versa) should be “relevant”, provided we generate with a well-trained language model. For instance, consider a random token sequence. This string would be irrelevant to most answers in our dataset and also (for good language models) have low sequence probability conditional to an answer.


